Universality in Freezing Cellular Automata

Cellular Automata have been used since their introduction as a discrete tool of modelization. In many of the physical processes one may modelize thus (such as bootstrap percolation, forest fire or epidemic propagation models, life without death, etc), each local change is irreversible. The class of freezing Cellular Automata (FCA) captures this feature. In a freezing cellular automaton the states are ordered and the cells can only decrease their state according to this "freezing-order". We investigate the dynamics of such systems through the questions of simulation and universality in this class: is there a Freezing Cellular Automaton (FCA) that is able to simulate any Freezing Cellular Automata, i.e. an intrinsically universal FCA? We show that the answer to that question is sensitive to both the number of changes cells are allowed to make, and geometric features of the space. In dimension 1, there is no universal FCA. In dimension 2, if either the number of changes is at least 2, or the neighborhood is Moore, then there are universal FCA. On the other hand, there is no universal FCA with one change and Von Neumann neighborhood. We also show that monotonicity of the local rule with respect to the freezing-order (a common feature of bootstrap percolation) is also an obstacle to universality.

==> localenergy.tex <==
A freezing-universal CAs can simulate all freezing CA of same dimension, but it can simulate CAs which are not freezing. For instance, a CA with states ${Q=\{0,\ldots,k\}\cup\{\iota\}}$ and neighborhood ${V=\{0,1\}}$ that increases or decreases the local state depending on the presence of $\iota$ in the context, defined by the local map: 
\[f(a,b) =
\begin{cases}
  \iota &\text{ if }a=\iota,\\
  \max(a+1,k) &\text{ else if }b=\iota,\\
  \min(a-1,0) &\text{ else.}
\end{cases}
\]
Such a CA is not freezing but can be simulated by a freezing CA (which can be seen directly, and is also a consequence of Theorem~\ref{thm:elefreezesimu} below). However it is straightforward to check that a freezing CA cannot simulate a CA where there is no bound on the number of state change per cell.

\newcommand\G{{\mathbb{Z}^d}}
 Given a CA ${F:Q^\G\rightarrow Q^\G}$, we say that ${e: Q^\G\rightarrow\{0,\ldots,k\}^\G}$ is an \emph{explicit local energy} for $F$ if it is a sliding block map, \textit{i.e.}
${\forall c\in Q^{\G},\forall z\in \mathbb{Z}^{d},\ e(c)_{z}=\lambda(c|_{z+N})}$ for some finite $N\subseteq\G$ and local map ${\lambda : Q^N\rightarrow\{0,\ldots,k\}}$,
and verifies ${\forall c\in Q^\G, \forall z\in\G}$:
\begin{itemize}
\item ${e(F(c))_z\leq e(c)_z}$\text{ and}
\item ${F(c)_z\neq c_z\Rightarrow  e(F(c))_z<e(c)_z}$.
\end{itemize}

An explicit local energy for some CA $F$ gives a proof that its cells can only change a bounded number of time their state. For instance, the example given above admits the following explicit local energy:
\[e(c)_z =
\begin{cases}
  0&\text{ if }c_z=\iota,\\
  c_z&\text{ else if }c_{z+1}\neq\iota,\\
  k-c_z&\text{ else}.
\end{cases}
\]
Such local energy maps are also naturally found in some classes of CA like $\FCA$ or nilpotent CAs (recall that $F$ is nilpotent if $F^n$ is a \emph{constant} map for some $n$).

\begin{lemma}
  \label{lem:eergy}
  Any freezing CA and any nilpotent CA admits an explicit local energy.
\end{lemma}

It turns out that we can characterize the set of CA that can be simulated by freezing CAs through the notion of explicit local energy.

\begin{theorem}
  \label{thm:elefreezesimu}
  A CA $F$ admits an explicit local energy if and only if it is context-sensitive simulated by a freezing CA $G$.
\end{theorem}
\begin{proof}
  First suppose that $F$ admits an explicit local energy ${e: Q^\G\rightarrow\{0,\ldots,k\}^\G}$. We consider $G$ over alphabet ${Q_G=Q\times\{0,\ldots,k\}\cup\{\epsilon\}}$, with neighborhood the union of that of $F$ and $e$, and defined as follows: 
  \begin{itemize}
  \item if $\epsilon$ is not in the neighborhood and the two components of states locally look like ${c\in Q^\G}$ and ${e(c)\in\{0,\ldots,k\}^\G}$ then the new state has components defined by ${F(c)}$ and ${e(F(c))}$;
  \item in any other case generate the state $\epsilon$.
  \end{itemize}
  Defining the order $\preceq$ on $Q_G$ by
  \begin{itemize}
  \item ${\epsilon\preceq(q,i)}$ for any ${q\in Q}$ and ${i\in\{0,\ldots,k\}}$;
  \item ${(q,i)\preceq(q',i')}$ if ${i<i'}$;
  \item ${x\preceq x}$ for any ${x\in Q_G}$,
  \end{itemize}
  it is straightforward to check that $G$ is $\preceq$-freezing. Let ${\phi : Q^\G\rightarrow (Q\times\{0,\ldots,k\})^\G}$ be the encoding defined by ${\phi(c)}$ equal to $c$ on the first component of states and $e(c)$ on the second, it is straightforward to check that ${\phi\circ F = G\circ \phi}$
  which shows that $G$ simulates $F$.

  To prove the converse direction of the theorem, suppose now that a freezing CA $G$ simulates a CA $F$ with slowdown ${T}$ and block size $m$. Since iterating and applying a grouping operation on a freezing CA gives a freezing CA, we can suppose without loss of generality that ${m=1}$ and ${T=1}$. That is to say the simulation holds through the encoding $\overline\phi$ coming from a local map ${\phi:Q_G^{V}\rightarrow Q_F}$ so that we have: ${\overline{\phi}(F(c))=G(\overline{\phi}(c))}$. Lemma~\ref{lem:eergy} ensures that $G$ admits an explicit local energy ${e:Q_G^\G\rightarrow \{0,\ldots,k\}^\G}$. One can check that ${e\circ\overline\phi : Q_F^V\rightarrow\{0,\ldots,k\}}$ is the local map of an explicit local energy $\Psi$ for $F$, indeed:
  \begin{itemize}
  \item ${\Psi(F(c))_z = e(\overline\phi(F(c))_z = e(G(\overline\phi(c)))_z\leq e(\overline\phi(c))_z = \Psi(c)_z}$;
  \item moreover, if ${F(c)_z\neq c_z}$ then the condition of local injectivity on $\phi$ (item 1 of Definition~\ref{def:contextsensitivesimu}) ensures that ${\overline\phi(F(c))_z\neq\overline\phi(c)_z}$ that is to say ${G(\overline\phi(c))_z\neq\overline\phi(c)_z}$. $e$ being an explicit local energy for $G$ we deduce that: ${e(G(\overline\phi(c)))_z< e(\overline\phi(c))_z}$ that is to say ${\Psi(F(c))_z <\Psi(c)_z}$.
  \end{itemize}
  % \[\phi\circ F = G'\circ \phi\]
  % where $\phi$ is the (context-sensitive) injective coding. Since $G$ admits an explicit energy, so does ${G':}$. 
\end{proof}

